Space-Time Shift Keying Aided OTFS Modulation for Orthogonal Multiple Access

Space-time shift keying-aided orthogonal time frequency space modulation-based multiple access (STSK-OTFS-MA) is proposed for reliable uplink transmission in high-Doppler scenarios. As a beneficial feature of our STSK-OTFS-MA system, extra information bits are mapped onto the indices of the active dispersion matrices, which allows the system to enjoy the joint benefits of both STSK and OTFS signalling. Due to the fact that both the time-, space- and DD-domain degrees of freedom are jointly exploited, our STSK-OTFS-MA achieves increased diversity and coding gains. To mitigate the potentially excessive detection complexity, the sparse structure of the equivalent transmitted symbol vector is exploited, resulting in a pair of low-complexity near-maximum likelihood (ML) multiuser detection algorithms. Explicitly, we conceive a progressive residual check-based greedy detector (PRCGD) and an iterative reduced-space check-based detector (IRCD). Then, we derive both the unconditional single-user pairwise error probability (SU-UPEP) and a tight bit error ratio (BER) union-bound for our single-user STSK-OTFS-MA system employing the ML detector. Furthermore, the discrete-input continuous-output memoryless channel (DCMC) capacity of the proposed system is derived. The optimal dispersion matrices (DMs) are designed based on the maximum attainable diversity and coding gain metrics. Finally, it is demonstrated that our STSK-OTFS-MA system achieves both a lower BER and a higher DCMC capacity than its conventional spatial modulation (SM) {and its orthogonal frequency-division multiplexing (OFDM) counterparts. As a benefit, the proposed system strikes a compelling BER vs. system complexity as well as BER vs. detection complexity trade-offs.

==> acronyms.tex <==
%
%acronyms

\newacronym{AWGN}{AWGN}{additive white Gaussian noise}

\newacronym{BABF}{BABF}{blind adaptive beamforming}

\newacronym{BER}{BER}{bit error ratio}

\newacronym{CW}{CW}{continuous wave}

\newacronym{CU}{CU}{control unit}

\newacronym{JML}{JML}{joint maximum-likelihood}

\newacronym{DPSK}{DPSK}{differential phase shift key}

\newacronym{PSK}{PSK}{phase shift key}

\newacronym{EM}{EM}{expectation maximization}

\newacronym{PDF}{PDF}{probability density function}

\newacronym{CSI}{CSI}{channel state information}

\newacronym{EPC}{EPC}{electronic product code}

\newacronym{RF}{RF}{radio frequency}

\newacronym{RIP}{RIP}{rotational invariance property}

\newacronym{RFID}{RFID}{radio frequency identification}

\newacronym{IC}{IC}{integrated circuit}

\newacronym{IoTs}{IoTs}{Internet of Things}

\newacronym{ULA}{ULA}{uniform linear array}

\newacronym{UHF}{UHF}{ultra high frequency}

\newacronym{OLS}{OLS}{ordinary least square}

\newacronym{QCQPs}{QCQPs}{quadratically constrained quadratic programs}

\newacronym{SDR}{SDR}{semidefinite relaxation}

\newacronym{SCA}{SCA}{successive convex approximation}

\newacronym{WET}{WET}{wireless energy transfer}

\newacronym{UWB}{UWB}{ultrawide bandwidth}

\newacronym{ToA}{ToA}{time-of-arrival}

\newacronym{PoA}{PoA}{phase-of-arrival}

\newacronym{DoA}{DoA}{direction-of-arrival}

\newacronym{RSS}{RSS}{received signal strength}

\newacronym{MSE}{MSE}{mean square error}

\newacronym{DoF}{DoF}{degree of freedom}

\newacronym{UAV}{UAV}{unmanned aerial vehicle}

\newacronym{CAMs}{CAMs}{cooperative awareness messages}

\newacronym{BS}{BS}{base station}

\newacronym{ID}{ID}{identification}

\newacronym{PL}{PL}{platoon leader}

\newacronym{PM}{PM}{platoon member}
\newacronym{PMs}{PMs}{platoon members}

\newacronym{a.k.a.}{a.k.a.}{also know as}

\newacronym{DPM}{DPM}{disconnected platoon member}

\newacronym{BaS}{BaS}{Braking and Stopping}

\newacronym{TAs}{TAs}{transmit antennas}

\newacronym{RAs}{RAs}{receive antennas}

\newacronym{3D}{3D}{three-dimensional}

\newacronym{ACK}{ACK}{acknowledgement}

\newacronym{V2V}{V2V}{vehicle-to-vehicle}

\newacronym{V2I}{V2I}{vehicle-to-infrastructure}

\newacronym{WLAN}{WLAN}{wireless local area network}

\newacronym{UAVs}{UAVs}{unmanned aerial vehicles}

\newacronym{ML}{ML}{machine learning}

\newacronym{TOA}{TOA}{time of arrival}

\newacronym{UWB}{UWB}{ultrawideband}

\newacronym{OBU}{OBU}{on-board unit}

\newacronym{LOS}{LOS}{line-of-sight}

\newacronym{RIB}{RIB}{rotational invariance beamforming}




















